Malign Overfitting: Interpolation Can Provably Preclude Invariance

Learned classifiers should often possess certain invariance properties meant to encourage fairness, robustness, or out-of-distribution generalization. However, multiple recent works empirically demonstrate that common invariance-inducing regularizers are ineffective in the over-parameterized regime, in which classifiers perfectly fit (i.e. interpolate) the training data. This suggests that the phenomenon of "benign overfitting", in which models generalize well despite interpolating, might not favorably extend to settings in which robustness or fairness are desirable. In this work we provide a theoretical justification for these observations. We prove that -- even in the simplest of settings -- any interpolating learning rule (with arbitrarily small margin) will not satisfy these invariance properties. We then propose and analyze an algorithm that -- in the same setting -- successfully learns a non-interpolating classifier that is provably invariant. We validate our theoretical observations on simulated data and the Waterbirds dataset.

==> sections/supp_positive_result_backup2.tex <==
\section{Analysis of \texorpdfstring{\Cref{alg:two_phase_learning}}{}}
In this section we prove that Algorithm~\ref{alg:two_phase_learning} indeed achieves a non-trivial robust error. The section is organized similarly to the proof of our negative result, we will begin with notation, assumptions and restatement of \Cref{alg:two_phase_learning} in \Cref{sec:pos_part_defs}. Then in \Cref{sec:pos_part_bounds} we prove the required concentration results which we will use to show the main claims in \Cref{sec:pos_part_main_proofs}\\
\subsection{Notation and Assumptions} \label{sec:pos_part_defs}
Denote the first-stage training set indices by $S$, where $|S|=N$ and second stage ``fine-tuning" set by $|D|=M$. Let us denote:
\begin{align*}
    \bar{\rvn}_e &= \frac{1}{N_{e}}\sum_{i\in{S_{e}}}{n_i}, ~ \bar{\rvm}_e = \frac{1}{M_{e}}\sum_{i\in{D_{e}}}{n_i}, ~ \bar{\rvm}_{e, 1} = \frac{1}{M_{e,1}}\sum_{i\in{D_{e,1}}}{n_i}.
\end{align*}
Models will be defined by
\begin{align*}
    \w_e :=\:& \frac{1}{N_e}{\sum_{i\in{S_e}}{y_i\x_i}} = \mu_c + \theta_e\mu_s + \bar{\rvn}_e, \quad e\in{\{1,2\}}, \\
    f_{\rvv}(x; S) =\:&~ \langle v_1\cdot\w_1 + v_2\cdot\w_2, \x \rangle.
\end{align*}
The Equalized Opportunity (EOpp) constraint is
\begin{align*}
    \hat{T}_1(f_\rvv; D, S) &= \hat{T}_2(f_\rvv; D), \\
    \hat{T}_e(f_\rvv; D, S) &= \frac{1}{M_{e,1}}\sum_{i\in{D_{e,1}}}{f_\rvv(\x_i)}.
\end{align*}
\begin{assumption}
We assume w.l.o.g $\theta_2 > \theta_1$, define $\Delta:=\theta_2-\theta_1 > 0$ and $r_{\mu} = \frac{\norm{\mu_s}}{\norm{\mu_c}} > 1$. We consider $r_\mu, \Delta$ as fixed numbers. That is, they do not depend on $N, d$ and other parameters of the problem. Also define $r:=\frac{\Delta\theta_{\max}}{\Delta + 4\theta_{\max}}$, where $\theta_{\max} := \mathrm{arg}{\max}\{|\theta_1|, |\theta_2|\} \leq 1$.
\end{assumption}
The following additional assumptions will be required for our concentration bounds and will lead to the conditions that eventually appear in \Cref{prop:positive_result_main}.
\begin{assumption} \label{ass:norm_constraints_pos_result}
Let $t > 0$ be a fixed user specified value, which we define later and will control the success probability of the algorithm. We will assume that for each $e \in{\{1,2\}}$ and some universal constants $c_c, c_{s} > 0$:
\begin{align*}
    %% Version with constants
    % \norm{\mu_s}^2 &\geq t\max\left\{\frac{2\sigma^2}{r^2 N_e}, \frac{128\sigma^2}{(r\Delta)^2M_{e,1}}, \frac{4c\sigma^2\sqrt{d}}{M_{e', 1}r\Delta} \right\} \\
    % \norm{\mu_c}^2 &\geq t\max\left\{\frac{1152\sigma^2}{\Delta^2N_e}, \frac{10368\sigma^2r^2_\mu}{\left( \Delta^2 M_{e,1} \right)} , \frac{(96\sigma r_{\mu})^2}{\Delta^2 M_e}, \frac{288c \sigma^2\sqrt{d}}{M_{e', 1}\Delta^2}, \frac{48 c \sigma^2 d}{M_{e'} \Delta} \right\}
    \norm{\mu_s}^2 &\geq t\sigma^2 c_s\max\left\{\frac{1}{r^2 N_e}, \frac{1}{(r\Delta)^2M_{e,1}}, \frac{\sqrt{d}}{M_{e, 1}r\Delta} \right\} \\
    \norm{\mu_c}^2 &\geq t\sigma^2 c_c\max\left\{\frac{1}{\Delta^2N_e}, \frac{r^2_\mu}{\left( \Delta^2 M_{e,1} \right)} , \frac{ r_{\mu}^2}{\Delta^2 M_e}, \frac{\sqrt{d}}{M_{e, 1}\Delta^2}, \frac{\sqrt{d}}{M_{e} \Delta} \right\}
    % \norm{\mu_s}^2 &\geq 2t\sigma^2 \max\left\{ \frac{1}{r^2 N_e}, 4\frac{1}{r\Delta^2 M_{e,1}} \right\} \\
    % \norm{\mu_c}^2 &\geq t\sigma^2 \left\{ \frac{\left(49r_{\mu}\right)^2}{\Delta^4 M_e} \right\} \\
    % \norm{\mu_c}^2 &\leq \frac{\sigma^2 d}{N_e}
\end{align*}
\end{assumption}

\textbf{Analyzing the EOpp constraint.} Writing the terms defined above in more detailed form gives:
\begin{align*}
    \epsilon_e(\rvv) =& \langle \bar{\rvm}_{e, 1}, v_1\left(\mu_c + \theta_1\mu_s + \bar{\rvn}_1\right) + v_2\left(\mu_c + \theta_2\mu_s + \bar{\rvn}_2\right) \rangle \\
    \delta_e(\rvv) =& \langle \bar{\rvm}_{e}, v_1\left(\mu_c + \theta_1\mu_s + \bar{\rvn}_1\right) + v_2\left(\mu_c + \theta_2\mu_s + \bar{\rvn}_2\right) \rangle \\
    \hat{T}_{e}(f_{\rvv}; D, S) =& (v_1 + v_2)\norm{\mu_c}^2 + (v_1\theta_1 + v_2\theta_2)\theta_e \norm{\mu_s}^2 + \\
    &\langle \mu_c + \theta_e\mu_s, v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle + \epsilon_e(\rvv)
\end{align*}
So the EOpp constraint is:
\begin{align} \label{eq:EOpp_constraint}
    v_1&\left[\theta_1\norm{\mu_s}^2 + \langle\bar{\rvn}_1, \mu_s\rangle\right]\theta_1 + v_2 \left[\theta_2\norm{\mu_s}^2 + \langle \bar{\rvn}_2, \mu_s \rangle\right] \theta_1 + \epsilon_1(\rvv) = \nonumber\\
    &v_1\left[\theta_1\norm{\mu_s}^2 + \langle\bar{\rvn}_1, \mu_s\rangle\right]\theta_2 + v_2 \left[\theta_2\norm{\mu_s}^2 + \langle \bar{\rvn}_2, \mu_s \rangle\right] \theta_2 + \epsilon_2(\rvv)
\end{align}

\begin{lemma} \label{lem:EOpp_unit_ball_intersection}
Consider all the solutions $\rvv = (v_1, v_2)$ that satisfy EOpp and have $\norm{\rvv}_\infty=1$. With probability $1$ there are exactly two such solutions $\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}$, where $\rvv_{\mathrm{pos}}=-\rvv_{\mathrm{neg}}$.
\end{lemma}
We will consider $\rvv_{\mathrm{pos}}$ as the solution that satisfies $v_{\mathrm{pos}, 1} + v_{\mathrm{pos}, 2} > 0$.
\begin{proof}
Is it easy to see that the EOpp constraint is a linear equation in $v_1, v_2$ and with probability $1$ the coefficients in this linear equations are nonzero. Therefore the solutions to this equation form a line in $\reals^2$ that passes through the origin. Consequently, this line intersects the $l_{\infty}$ unit ball at two points, that we denote $\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}$, which are negations of one another.
\end{proof}

% We can also write the EOpp constraint with the ratio of $v_2 / v_1$ as follows (which is well-defined with probability $1$):
% \begin{align} \label{eq:EOpp_constraint}
% \frac{v_2}{v_1} = \frac{\left[\theta_1\norm{\mu_s}^2 + \langle \bar{\rvn}_1, \mu_s \rangle\right](\theta_2-\theta_1) + \langle \bar{\rvm}_{1, 1} - \bar{\rvm}_{2, 1}, \mu_c + \theta_1\mu_s + \bar{\rvn}_1 \rangle}{\left[\theta_2\norm{\mu_s}^2 + \langle \bar{\rvn}_2, \mu_s \rangle\right](\theta_1-\theta_2) + \langle \bar{\rvm}_{2, 1} - \bar{\rvm}_{1, 1}, \mu_c + \theta_2\mu_s + \bar{\rvn}_2 \rangle}
% \end{align}
% This should concentrate nicely around $-\frac{\theta_1}{\theta_2}$ (but we shall discuss concentration later). For now, let us denote the RHS by $c$ for convenience (abusing notation by dropping the dependence on all the parameters) and characterize our solutions.

\textbf{The proposed algorithm.} Now we can restate our algorithm in terms of $v_{\mathrm{pos}}$ and $v_{\mathrm{neg}}$ and analyze its retrieved solution.
\begin{algorithm}[t]
\onehalfspacing
\caption{Two Phase Learning of Overparameterized Invariant Classifiers: With $\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}$}
\label{alg:two_phase_learning_ver_b}
\begin{algorithmic}
\Require Datasets $(S_1, S_2)$ %$\{(\x_i, y_i)\}_{i=1}^{N}$ and a partition $S_1, S_2$ into environments. 
and an invariance constraint function family $\F(\cdot, \cdot)$
\Ensure A classifier $f_{\rvv}(\x)$
\State Draw subsets of data without replacement $S^{\mathrm{trn}}_e\subset S_e$ for $e\in{\{1,2\}}$ where $\left | S^{\mathrm{trn}}_e \right| = N_e / 2$
\State Stage 1: %Calculate $\w^e_{\mathrm{mean}}$, the signed-sample-mean model (see \defref{def:w_avg}) over $S^{\mathrm{trn}}_e$. \yc{$\w^e_{\mathrm{mean}}$ seems to be inconsistent with $\w_e$ in the proof sketch. I like the latter better}
Calculate 
$\w_e= 2N_e^{-1}\sum_{(\x, y)\in{S^{\mathrm{trn}}_e}}{\x y}$ for each $e\in{\{1,2\}}$
\State Define $S_e^{\mathrm{fine}} = S_e \setminus S_e^{\mathrm{trn}}$ for $e\in{\{1, 2\}}$ and $S^{\mathrm{fine}} = S_1^{\mathrm{fine}} \cup S_2^{\mathrm{fine}}$
\State Consider the solutions $\{\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}\}$ that satisfy EOpp and also $\norm{\rvv}_\infty=1$.
\State Stage 2: Return
%$f_{\rvv}(\x; S_{\mathrm{trn}}) = \inp{v_1\cdot(2N_1)^{-1}\w^{1}_{\mathrm{mean}} + v_2\cdot(2N_2)^{-1}\w^2_{\mathrm{mean}}}{\x}$ 
$f_{\rvv^*}(\x) = \inp{v^*_1\cdot\w_1 + v^*_2\cdot \w_2}{\x}$ 
that solves
%\begin{align*}
%    \maximize_{\norm{\rvv}_{\infty}=1} & \sum_{i\in{S^{\mathrm{fine}}}}{f_{\rvv}(\x_i)y_i } \\    &\text{subject to }\ f_\rvv\in{\F(S^{\mathrm{fine}})}.
%\end{align*}
\begin{equation*}
  \maximize_{\rvv\in{\{\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}\}}} \sum_{(\x,y)\in{S^{\mathrm{fine}}}}{f_{\rvv}(\x)y } % \quad\text{subject to}\quad {\norm{\rvv}_{\infty}=1} \quad\text{and}\quad  f_\rvv\in{\F(S_1^{\mathrm{fine}}, S_2^{\mathrm{fine}})}
\end{equation*}
\end{algorithmic}
\end{algorithm}
% \begin{itemize}
%     \item Calculate $\w_1$ and $\w_2$ according to their definitions.
%     \item Consider the solutions $\{\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}\}$ that satisfy EOpp and also $\norm{\rvv}_\infty=1$.
%     \item Return the solution: $\rvv\in{\{\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}\}}$ which has the higher score, where the score is:
%     \begin{align*}
%       \rvv^* \in{\mathrm{arg}\max_{\rvv\in{\{\rvv_{\mathrm{pos}}, \rvv_{\mathrm{neg}}\}}}{\sum_{i\in{D}}{ \langle v_1\w_1 + v_2\w_2, y_i\x_i \rangle}}}
%     \end{align*}
% \end{itemize}

\subsection{Required Concentration Bounds} \label{sec:pos_part_bounds}
We now turn to prove concentration bounds that we shall use to finalize our argument regarding \Cref{alg:two_phase_learning_ver_b}.
Note that $\rvv^*$ is determined by all the other random factors in the problem, hence we should be careful when using $\rvv^*$ in our bounds. We will only use the fact that $\norm{\rvv^*}_\infty = 1$ and hence $\norm{\rvv^*}_1 \leq 2$.

To bound the inner product of noise vectors, we use \cite[Theorem 1.1]{rudelson2013hanson}:
\begin{theorem} (Hanson-Wright inequality). Let $X=\left(X_1, \ldots, X_n\right) \in \mathbb{R}^n$ be a random vector with independent components $X_i$ which satisfy $\mathbb{E} X_i=0$ and $\left\|X_i\right\|_{\psi_2} \leq$ $K$. Let $A$ be an $n \times n$ matrix. Then, for every $t \geq 0$,
$$
\mathbb{P}\left(\left|X^{\top} A X-\mathbb{E}[ X^{\top} A X\right]|>t\right) \leq 2 \exp \left[-c \min \left(\frac{t^2}{K^4\|A\|_{\mathrm{HS}}^2}, \frac{t}{K^2\|A\|}\right)\right].
$$
\end{theorem}
We can apply this theorem to get the following result.
\begin{corollary} \label{corr:noises_inner_prod}
There exists a universal constant $c>0$ such that for any $e\in{\{1,2\}}$ and $e'\in{\{1,2\}}$ (when we assume w.l.o.g that $M_{e'} \leq N_e$),
\begin{align} \label{eq:noise_inprod_bnd}
\sP \left( | \langle \bar{\rvn}_e, \bar{\rvm}_{e'} \rangle | > t \right) \leq 2\exp\left[ -c \min\left(\frac{M_{e'}^2 t^2}{\sigma^4 d}, \frac{M_{e'} t}{\sigma^2\sqrt{d}}\right) \right].
\end{align}
\end{corollary}
\begin{proof}
We take $X$ as the concatenation of $\bar{\rvn}_e$ and $\bar{\rvm}_{e'}$, then $A$ is set such that $X^\top A X = \langle \bar{\rvn}_e, \bar{\rvm}_{e'} \rangle$ (e.g. $A_{i, i+d}=1$ for $1 \leq i \leq d$ and $0$ elsewhere).
Then $\norm{A}_{HS}^2 = d$ and $\norm{A}=\sqrt{d}$. Since entries in $\bar{\rvn}_e, \bar{\rvm}_{e'}$ are distributed as $\N(0, \frac{\sigma^2}{N_e}), \N(0, \frac{\sigma^2}{M_e})$ respectively, we have $K \leq C \frac{\sigma}{\sqrt{\min{\{N_e, M_{e'}\}}}}$ for some universal constant $C$ which we can incorporate into the constant $c$ in the theorem. Since we assumed w.l.o.g that $M_{e'} < N_e$, this gives:
\begin{align*}
    \sP \left( | \langle \bar{\rvn}_e, \bar{\rvm}_{e'} \rangle | > t \right) \leq 2\exp\left[ -c \min\left(\frac{M_{e'}^2 t^2}{\sigma^4 d}, \frac{M_{e'} t}{\sigma^2\sqrt{d}}\right) \right].
\end{align*}
\end{proof}

The next statement collects all of the concentration results we require for the other parts of the proof.
\begin{lemma} \label{lem:positive_result_concentrations}
Define $r:= \frac{\Delta \theta_{\max}}{\Delta + 4\theta_{\max}}$ where $\theta_{\max}:=\mathrm{arg}\max_{e\in{\{1,2\}}}\{|\theta_e|\}$, denote by $\rvv^*$ the solution retrieved by \Cref{alg:two_phase_learning_ver_b}, and let $t>0$. When \assumref{ass:norm_constraints_pos_result} holds,
then with probability at least \succesprobpos we have that all the following events occur simultaneously (for all $e,e'\in{\{1, 2\}}$):
\begin{align}
    |\langle \bar{\rvn}_e, \mu_s \rangle| \leq& r \norm{\mu_s}^2 \label{eq:n_mu_assum}\\
    |\langle \bar{\rvn}_e, \mu_c \rangle| \leq& \frac{\Delta}{24} \norm{\mu_c}^2 \label{eq:n_muc_assum}\\
    |\langle \bar{\rvm}_{e,1}, \mu_c + \theta_{e'}\mu_s \rangle| \leq& \min \left\{ \frac{1}{4} r \Delta \norm{\mu_s}^2, \frac{\Delta}{36}\norm{\mu_c}^2 \right\} \label{eq:m_mus_assum}\\
    |\langle \bar{\rvm}_{e,1}, \mu_s  \rangle| \leq& \frac{\Delta}{64}\norm{\mu_c}^2 \label{eq:m_mu_spu_assum}\\
    |\langle \bar{\rvn}_e, \bar{\rvm}_{e',1} \rangle| \leq& \min\left\{\frac{1}{4} r\Delta \norm{\mu_s}^2, \frac{\Delta^2}{288} \norm{\mu_c}^2\right\} \label{eq:noise_prod_assum} \\
    \left| \langle \bar{\rvm}_e, \left(\mu_c + \theta_{e'}\mu_s\right) \rangle \right| \leq& \frac{1}{48}\Delta\cdot{\norm{\mu_c}}^2  \label{eq:m_mus_assum2}\\
    \left| \langle \bar{\rvn}_e, \bar{\rvm}_{e'} \rangle \right| \leq& \frac{1}{48}\Delta\cdot{\norm{\mu_c}}^2 \label{eq:noise_prod_assum2} \\
    \norm{\bar{\rvn}_e} \leq& t \sqrt{\frac{2\sigma^2 d}{N_e}} \label{eq:noise_norm_assum}
\end{align}
\end{lemma}
\begin{proof}

We first treat \eqref{eq:n_mu_assum} with a tail bound for Gaussian variables,
\begin{align*}
    \langle \bar{\rvn}_e, \mu_s
    \rangle \sim \N (0, \frac{\sigma^2\norm{\mu_s}^2}{N_e}) \Rightarrow \sP\left(|\langle \bar{\rvn}_e, \mu_s\rangle| > t_2 \right) \leq 2\exp\left( -\frac{t_2^2 N_e}{2\sigma^2\norm{\mu_s}^2} \right).
\end{align*}
Hence as long as $\norm{\mu_s}^2 \geq t\frac{2\sigma^2}{r^2 N_e}$, \eqref{eq:n_mu_assum} holds with probability at least $1-4\exp\{-t^2\}$ (since we take a union bound on the two environments). Following the same inequality and taking a union bound, if $\norm{\mu_c}^2 \geq t\frac{1152\sigma^2}{\Delta^2N_e}$, \eqref{eq:n_muc_assum} and \Cref{eq:n_mu_assum} hold simultaneously with probability at least $1-8\exp\{-t^2\}$.

We use the same bound for \eqref{eq:m_mus_assum}, \eqref{eq:m_mu_spu_assum} and \eqref{eq:m_mus_assum2} while using $|\theta_e|\leq 1$. Hence for $t_2=\frac{1}{4} r \Delta \cdot \norm{\mu_s}^2$ and $t_2=\frac{1}{36}\Delta\cdot\norm{\mu_c}^2$,
\begin{align*}
    \sP\left(|\langle \bar{\rvm}_{e,1}, \mu_c + \theta_{e'}\mu_s \rangle| > t_2 \right) &\leq 2\exp\left( -\frac{t_2^2 M_{e,1}}{2\sigma^2\norm{\mu_c + \theta_{e'}\mu_s}^2} \right) = 2\exp\left( -\frac{(r\Delta)^2\norm{\mu_s}^4 M_{e,1}}{32\sigma^2\norm{\mu_c + \theta_{e'}\mu_s}^2} \right) \\
    &\leq 2\exp\left( -\frac{(r\Delta)^2\norm{\mu_s}^2 M_{e,1}}{128\sigma^2} \right), \\
    \sP\left(|\langle \bar{\rvm}_{e,1}, \mu_c + \theta_{e'}\mu_s \rangle| > t_2 \right) &\leq 2\exp\left( -\frac{\Delta^2 \norm{\mu_c}^4 M_{e,1}}{2592\sigma^2\norm{\mu_c + \theta_{e'}\mu_s}^2} \right) = 2\exp\left( -\frac{\Delta^2 \norm{\mu_c}^2 M_{e,1}}{10368\sigma^2r^2_\mu} \right).
\end{align*}
Similarly with $t_2 = \frac{1}{48}\Delta\cdot\norm{\mu_c}^2$,
\begin{align*}
    \sP\left( \left| \langle \bar{\rvm}_e, \left(\mu_c + \theta_{e'}\mu_s\right) \rangle \right| > t_2 \right) \leq 2\exp\left( -\frac{\Delta^2\norm{\mu_c}^4 M_{e}}{(48\sigma\norm{\mu_c + \theta_{e'}\mu_s})^2} \right).
\end{align*}
Taking the required union bounds we get that with probability at least $1-24\exp{\left( -t^2 / 2 \right)}$ \eqref{eq:m_mus_assum}, \eqref{eq:m_mu_spu_assum} and \eqref{eq:m_mus_assum2} hold, as long as $\norm{\mu_s}^2 \geq t\cdot 128\sigma^2((r\Delta)^2 M_{e,1})^{-1}$ and $\norm{\mu_c}^2 \geq t\cdot\max\left\{10368\sigma^2r^2_\mu\left( \Delta^2 M_{e,1} \right)^{-1} , (96\sigma r_{\mu})^2(\Delta^2 M_e)^{-1}\right\}$.

For \eqref{eq:noise_prod_assum} and \eqref{eq:noise_prod_assum2} we use \corref{corr:noises_inner_prod}: \footnote{For simplicity, assume we have $\sqrt{M_{1,1}^{-2} + M_{2,1}^{-2}} \leq N^{-1}_1$ and that we set $t$ large enough such that $\left(M_{1,1}^{-1} + M_{2,1}^{-1}\right)^{-2}t^2 / (\sigma^4 d) \geq \left(M_{1,1}^{-1} + M_{2,1}^{-1}\right)^{-1}t / (\sigma^2 \sqrt{d})$}
\begin{align*}
    \sP\left( |\langle \bar{\rvn}_e, \bar{\rvm}_{e',1} \rangle| \geq t_2  \right) \leq 2\exp \left[ -c \frac{M^2_{e', 1}t_2^2}{\sigma^4 d} \right]
\end{align*}
Setting $t_2=\frac{r\Delta}{4}\norm{\mu_s}^2$ or $t_2=\frac{\Delta^2}{288}\norm{\mu_c}^2$ we will get that:
\begin{align*}
    &\sP\left( |\langle \bar{\rvn}_e, \bar{\rvm}_{e',1} \rangle| \geq \min\left\{ \frac{r\Delta}{4}\norm{\mu_s}^2,  \frac{\Delta^2}{288}\norm{\mu_c}^2\right\} \right) \leq \\
    &\qquad\qquad 2\exp\left( -c\frac{M^2_{e',1}}{\sigma^4 d} \min \left\{ \frac{(r\Delta)^2}{16}\norm{\mu_s}^4, \frac{\Delta^4}{288^2}\norm{\mu_c}^4\right\} \right)
\end{align*}
Hence we require $\norm{\mu_c}^2 \geq t\cdot c \cdot(M_{e', 1}\Delta^2)^{-1}\cdot(288 \sigma^2\sqrt{d})$ and $\norm{\mu_s}^2 \geq t\cdot c \cdot(M_{e', 1}r\Delta)^{-1}\cdot(4 \sigma^2\sqrt{d})$ for \eqref{eq:noise_prod_assum} to hold. For \eqref{eq:noise_prod_assum2} we can get in a similar manner that it holds in case that $\norm{\mu_c}^2 \geq t \cdot c \cdot (M_{e'} \Delta)^{-1}(48\sigma^2 \sqrt{d})$. The probability for all the events listed so far to occur is at least $1-32\exp\left(-t^2/2\right)$. Finally, for \eqref{eq:noise_norm_assum} we simply use the bound on a norm of Gaussian vector:
\begin{align*}
    \sP\left( \norm{\bar{\rvn}_e} \geq t_2\right) \leq 2\exp\left(-\frac{t_2^2N_e}{2\sigma^2 d}\right)
\end{align*}
Plugging in $t\sqrt{\frac{2\sigma^2 d}{N_e}}$ we arrive at the desired result with a final union bound that give the overall probability of at least $1-34\exp\left(-t^2/2\right)$.
\end{proof}

We now use the bounds above to write down specific bounds on expressions that we use during the subsequent proof.
\begin{corollary} \label{corro:positive_result_required_events}
Conditioned on all the events in \lemref{lem:positive_result_concentrations}, we have for $e\in{\{1,2\}}$ that:
\begin{align}
\frac{\Delta}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2 &\geq |\epsilon_2(\rvv) - \epsilon_1(\rvv)| \label{eq:event_corro_eq1}\\
\frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2 &\geq |\langle \mu_c , v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2\rangle| \label{eq:event_corro_eq2}\\
\frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2 &\geq |\langle \bar{\rvm}_e, (v_1+v_2)\mu_c + (\theta_1v_1 + \theta_2v_2)\mu_s + v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle | \label{eq:event_corro_eq3}\\
r\Delta \norm{\mu_s}^2 &\geq |\langle \bar{\rvm}_{1,1} - \bar{\rvm}_{2,1}, \mu_c + \theta_e\mu_s + \bar{\rvn}_e \rangle| \label{eq:event_corro_eq4}\\
r \norm{\mu_s}^2 &\geq |\langle\bar{\rvn}_e, \mu_s\rangle| \label{eq:event_corro_eq5}\\
5t\sqrt{\frac{\sigma^2 d}{\min_e{N_e}}} &\geq \norm{\w} \label{eq:event_corro_eq6}
\end{align}
\end{corollary}

\begin{proof}
\eqref{eq:event_corro_eq5} is just \eqref{eq:n_mu_assum} restated for convenience. \eqref{eq:event_corro_eq4} is a combination of \eqref{eq:m_mus_assum} and \eqref{eq:noise_prod_assum}:
\begin{align*}
    |\langle \bar{\rvm}_{1,1} - \bar{\rvm}_{2,1}, \mu_c + \theta_e\mu_s + \bar{\rvn}_e \rangle| \leq \sum_{e'} | \langle \bar{\rvm}_{e',1}, \mu_c + \theta_e\mu_s \rangle | + | \langle \bar{\rvm}_{e',1}, \bar{\rvn}_e \rangle| \leq r\Delta\norm{\mu_s}^2
\end{align*}
These are the events required for \lemref{lem:v_sum_bound}, hence from now on we can now assume that:
\begin{align*}
    |v_1 + v_2| \geq \frac{\Delta}{2} = \frac{\Delta}{4}\cdot 2 \geq \frac{\Delta}{4}\norm{\rvv}_1
\end{align*}
Now we can combine with \eqref{eq:n_muc_assum} to prove \eqref{eq:event_corro_eq2}:
\begin{align*}
    \langle \mu_c, v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle \leq \sum_{e}{|v_e|\cdot|\langle \mu_c, \bar{\rvn}_e \rangle|} \leq \norm{\rvv}_1 \frac{\Delta}{24}\norm{\mu_c}^2 \leq \frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2
\end{align*}
Next we prove \eqref{eq:event_corro_eq3} in a similar manner using \eqref{eq:m_mus_assum2} and \eqref{eq:noise_prod_assum2}:
\begin{align*}
    |\langle \bar{\rvm}_e,& (v_1+v_2)\mu_c + (\theta_1v_1 + \theta_2v_2)\mu_s + v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle| \leq \\
    &\sum_{e'}{|v_{e'}|\cdot\left(|\langle \bar{\rvm}_e, \mu_c + \theta_{e'}\mu_s \rangle| + |\langle \bar{\rvm}_e, \bar{\rvn}_{e'} \rangle|\right)} \leq \norm{\rvv}_1\cdot 2\cdot\frac{1}{48}\Delta\norm{\mu_c}^2 \leq \frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2
\end{align*}

For \eqref{eq:event_corro_eq1}, let us write the right hand side:
\begin{align*}
\left| \epsilon_2(\rvv) - \epsilon_1(\rvv) \right| &= \left| \langle \bar{\rvm}_{2,1}-\bar{\rvm}_{1,1}, v_1(\mu_c + \theta_1\mu_s +\bar{\rvn}_1) + v_2(\mu_c + \theta_2\mu_s +\bar{\rvn}_2) \rangle \right| \\
& = |(v_1 + v_2)\cdot\langle \bar{\rvm}_{2,1}-\bar{\rvm}_{1,1}, \mu_c + \half(\theta_1+\theta_2)\mu_s \rangle \\
& + \langle \bar{\rvm}_{2,1}-\bar{\rvm}_{1,1}, v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle + \half(v_1-v_2)\langle \bar{\rvm}_{2,1}-\bar{\rvm}_{1,1}, \Delta\mu_s \rangle| \\
& \leq |v_1 + v_2|\cdot\sum_{e}{|\langle \bar{\rvm}_{e,1}, \mu_c + \half(\theta_1+\theta_2\mu_s) \rangle|} + \norm{\rvv}_1\sum_{e,e'}{|\langle \bar{\rvm}_{e,1}, \bar{\rvn}_{e'} \rangle|} \\
& + \half \Delta \norm{\rvv}_1 \sum_{e}{|\langle \bar{\rvm}_{e,1}, \mu_s  \rangle|} \\
& \leq |v_1 + v_2|\cdot\sum_{e}{|\langle \bar{\rvm}_{e,1}, \mu_c + \half(\theta_1+\theta_2\mu_s) \rangle|} + \frac{4}{\Delta}|v_1 + v_2|\sum_{e,e'}{|\langle \bar{\rvm}_{e,1}, \bar{\rvn}_{e'} \rangle|} \\
& + 2 |v_1 + v_2| \sum_{e}{|\langle \bar{\rvm}_{e,1}, \mu_s  \rangle|} \\
&\leq \frac{1}{6}\Delta|v_1 + v_2|
\end{align*}
The first inequality is simply a triangle inequality, the second plugs in the bound we obtained for $\norm{\rvv}_1$ and the last uses the relevant inequalities from \lemref{lem:positive_result_concentrations}.

For \eqref{eq:event_corro_eq6}, we write the weights of the returned linear classifier as:
\begin{align*}
    \w = v^*_1(\mu_c + \theta_1\mu_s + \bar{\rvn}_1) + v^*_2(\mu_c + \theta_2\mu_s + \bar{\rvn}_2)
\end{align*}
Hence we can bound:
\begin{align*}
\norm{\w} -& (v^*_1+v^*_2) \norm{\mu_c} \leq \norm{(v^*_1\theta_1 + v^*_2\theta_2)\mu_s + v^*_1\bar{\rvn}_1 + v^*_2\bar{\rvn}_2} \\
&= \sqrt{(v_1^*\theta_1 + v_2^*\theta_2)^2\norm{\mu_s}^2 + 2\langle v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2 , (v_1^*\theta_1 + v_2^*\theta_2)\mu_s \rangle + \norm{v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2}^2} \\
&=\sqrt{(v_1^*\theta_1 + v_2^*\theta_2)\left((v_1^*\theta_1 + v_2^*\theta_2)\norm{\mu_s}^2 + 2\langle v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_1, \mu_s \rangle\right) + \norm{v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2}^2}
\end{align*}
We also proved in \lemref{lem:retrieved_solution}, that under the events we assumed and the EOpp constraint:
\begin{align*}
    (v_1^*\theta_1 + v_2^*\theta_2)\norm{\mu_s}^2 + 2\langle v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2, \mu_s \rangle &\leq 2\left((v_1^*\theta_1 + v_2^*\theta_2)\norm{\mu_s}^2 + |\langle v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2, \mu_s \rangle|)\right) \\
    &\leq \frac{1}{3}(v_1^* + v_2^*)\norm{\mu_c}^2
\end{align*}
Incorporating with $v_1^*\theta_1 + v_2^*\theta_2 \leq 2(v_1^* + v_2^*)$, the concavity of the square root and \eqref{eq:noise_norm_assum}, we get:
\begin{align*}
    \norm{\w} &\leq \left(1 + \sqrt{2 / 3}\right)(v_1^* + v_2^*)\norm{\mu_c} + \norm{v_1^*\bar{\rvn}_1 + v_2^*\bar{\rvn}_2} \\
    &\leq \left(1 + \sqrt{2 / 3}\right)(v_1^* + v_2^*)\norm{\mu_c} + \norm{\bar{\rvn}_1} + \norm{\bar{\rvn}_2} \\
    &\leq \left(1 + \sqrt{2 / 3}\right)(v_1^* + v_2^*)\norm{\mu_c} + t\cdot\sqrt{\frac{\sigma^2 d}{\min_e{N_e}}} \\
    &\leq 4\norm{\mu_c} + t\cdot\sqrt{\frac{\sigma^2 d}{\min_e{N_e}}} \\
    &\leq 5t\cdot\sqrt{\frac{\sigma^2 d}{\min_e{N_e}}}
\end{align*}
\end{proof}

\subsection{Proofs of Main Result}\label{sec:pos_part_main_proofs}
We first analyze the two possible solutions $v_{\mathrm{pos}}$ and $v_{\mathrm{neg}}$ and show that their coordinates cannot be negations of each other. Intuitively, in an ideal scenario with infinite data, the EOpp constraint will enforce $v_1\theta_1 = -v_2\theta_2$. Then $v_1=-v_2$ is only possible if $\theta_1=\theta_2$, which we assume is not the case (if it is, we cannot identify the spurious correlation from data). The assumption of a fixed $\Delta>0$, will let us show that indeed with high probability $v_1=-v_2$ does not occur.
\begin{lemma} \label{lem:v_sum_bound}
Let $t>0$ and consider the solutions $v_{\mathrm{neg}},v_{\mathrm{pos}}$ that the algorithm may return. With probability at least \succesprobpos, the solutions satisfy $|v_1 + v_2| \geq \frac{\Delta}{2}$.
\end{lemma}
\begin{proof}
Assume that for $e\in{\{1, 2\}}$ the following events occur:
\begin{align} \label{eq:expected_loss_assum1}
|\langle\bar{\rvn}_e, \mu_s\rangle| &\leq r \norm{\mu_s}^2 \\
\label{eq:expected_loss_assum2}
|\langle \bar{\rvm}_{1,1} - \bar{\rvm}_{2,1}, \mu_c + \theta_e\mu_s + \bar{\rvn}_e \rangle| &\leq r\Delta \norm{\mu_s}^2
\end{align}

\corref{corro:positive_result_required_events} will show that they occur with the desired probability in our statement. Let us incorporate these events into the EOpp constraint. We group the items multiplied by $v_1$ and those multiplied by $v_2$:
\begin{align*}
    -v^*_1\big[\theta_1\norm{\mu_s}^2\Delta + \langle\bar{\rvn}_1, \mu_s\rangle&\Delta + \langle \bar{\rvm}_{1,1} - \bar{\rvm}_{2,1}, \mu_c + \theta_1\mu_s + \bar{\rvn}_1 \rangle \big] = \\
    & v^*_2 \left[\theta_2\norm{\mu_s}^2\Delta + \langle \bar{\rvn}_2, \mu_s \rangle \Delta + \langle \bar{\rvm}_{2,1} - \bar{\rvm}_{1,1}, \mu_c + \theta_2\mu_s + \bar{\rvn}_2 \rangle \right]
\end{align*}

Let us denote for convenience (where we drop the dependence on parameters in the notation):
\begin{align*}
    a = \norm{\mu_s}^{-2}\Delta \left( \langle\bar{\rvn}_1, \mu_s\rangle + \Delta^{-1}\langle \bar{\rvm}_{1,1} - \bar{\rvm}_{2,1}, \mu_c + \theta_1\mu_s + \bar{\rvn}_1 \rangle\right) \\
    b = \norm{\mu_s}^{-2}\Delta \left( \langle\bar{\rvn}_2, \mu_s\rangle + \Delta^{-1}\langle \bar{\rvm}_{2,1} - \bar{\rvm}_{1,1}, \mu_c + \theta_2\mu_s + \bar{\rvn}_2 \rangle\right)
\end{align*}
Now the EOpp constraint can be written as $-v_1^*\norm{\mu_s}^2\Delta\left( \theta_1 + a \right) = v_2^*\norm{\mu_s}^2\Delta\left( \theta_2 + b \right)$. Plugging in \eqref{eq:expected_loss_assum1} and \eqref{eq:expected_loss_assum2}, we see that $\max\{ |a|, |b| \} \leq r$.

Assume that $|\theta_1 + b| \geq |\theta_2 + a|$,
and note that since $\norm{\rvv^*}_\infty=1$ we have that $|v_1^*| = 1$ (the proof for the other case is analogous). \footnote{In the case where $|\theta_2 + a| \geq |\theta_1 + b|$ then $|v_2^*| = 1$ would hold.} We note that by definition $\Delta \leq 2\theta_{\max}$, hence if $v_2^*=0$ we have $|v_1^* + v_2^*| = 1 \geq \frac{\Delta}{2\theta_{\max}}$ and our claim holds. Otherwise, we can write:
\begin{align*}
    |v_1^* + v_2^*| &= \left|1 -\frac{\theta_2+b}{\theta_1+a}\right| = \left| \frac{\Delta + a - b}{\theta_1 + a} \right| \geq \frac{\Delta - 2r}{\theta_{\max} + r} = \frac{\Delta - 2\frac{\Delta\theta_{\max}}{\Delta + 4\theta_{\max}}}{\theta_{\max} + \frac{\Delta\theta_{\max}}{\Delta + 4\theta_{\max}}} \\
    &= \frac{\Delta\left(\Delta + 4\theta_{\max} - 2\theta_{\max}\right)}{\theta_{\max}\left(\Delta + 4\theta_{\max} + \Delta\right)} = \frac{\Delta}{2\theta_{\max}} \geq \frac{\Delta}{2}
\end{align*}
\end{proof}
The result above will be useful for proving the rest of our claims towards the performance guarantees of the algorithm. We first show that the retrieved solution is the one that is positively aligned with $\mu_c$.

\begin{lemma} \label{lem:retrieved_solution}
With probability at least \succesprobpos, between the two solutions considered at the second stage of our algorithm, the one with $v_1 + v_2 \geq 0$ achieves a higher score.
\end{lemma}
\begin{proof}
    Let's write down the score on environment $e\in{\{1, 2\}}$ in detail:
    \begin{align} \label{eq:emp_score_decompose}
       \sum_{i\in{D_e}}{\w^\top \x_i y_i} =& (v_1+v_2)\norm{\mu_c}^2 + \langle \mu_c , v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2\rangle + \\ & (v_1\theta_1 + v_2\theta_2)\theta_e\norm{\mu_s}^2 + \langle \mu_s, \theta_e\left(v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2\right) \rangle + \nonumber \\
       &\langle \bar{\rvm}_e, (v_1+v_2)\mu_c + (\theta_1v_1 + \theta_2v_2)\mu_s + v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle \nonumber
    \end{align}
We will bound all the items other than $(v_1 + v_2)\norm{\mu_s}^2$ with concentration inequalities, and for the second line also use the EOpp constraint. Regrouping items in \eqref{eq:EOpp_constraint} we have:
\begin{align*}
    \left| \left(v_1\theta_1 + v_2\theta_2\right) \norm{\mu_s}^2 + \langle \mu_s, v_1\bar{\rvn}_1 + v_2\bar{\rvn}_2 \rangle \right|\cdot \Delta = |\epsilon_2(\rvv) - \epsilon_1(\rvv)|
\end{align*}
In \corref{corro:positive_result_required_events} we will prove that with probability at least \succesprobpos, it holds that $|\epsilon_2(\rvv) - \epsilon_1(\rvv)| \leq \frac{\Delta}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2$. Combined with $|\theta_e| < 1$, we get that the magnitude of the terms in the second line of \eqref{eq:emp_score_decompose} is bounded by $\frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2$. We will also show in \corref{corro:positive_result_required_events} that the other two terms in \eqref{eq:emp_score_decompose} besides $(v_1 + v_2)\norm{\mu_c}^2$, are bounded by $\frac{1}{6}|v_1 + v_2|\cdot\norm{\mu_c}^2$. Hence we have for some $b$ such that $|b| \leq \half |(v_1 + v_2)|\cdot\norm{\mu_c}^2$ that:
\begin{align*}
    \sum_{i\in{D_e}}{\w^\top \x_i y_i} = (v_1 + v_2)\norm{\mu_c}^2 + b
\end{align*}
We note that the score in the algorithm is a weighted average of the scores over the training environments, yet the derivation above holds regardless of $e$. That is, $\theta_e$ did not play a role in the derivation other than the assumption that its magnitude is smaller than $1$. Hence it is clear that the solution $\rvv^*=\rvv_{\mathrm{pos}}$ will be chosen over $\rvv_{\mathrm{neg}}$.
\end{proof}

Once we have characterized our returned solution, it is left to show its guaranteed performance over all environments $\theta \in{[-1, 1]}$. We can draw a similar argument to \lemref{lem:retrieved_solution} to reason about the expected score obtained in each environment.
\begin{lemma}\label{lem:expected_score}
Let $t>0$ and consider the retrieved solution $\rvv^*$. With probability at least \succesprobpos,
the expected score of $\rvv^*$ over any environment corresponding to $\theta\in{[-1, 1]}$ is larger than $\frac{\Delta}{3}\norm{\mu_c}^2$.
\end{lemma}
\begin{proof}
The expected score can be written same as in \eqref{eq:emp_score_decompose}, except we can drop the last item since it has expected value $0$. We let $\theta\in{[-1, 1]}$ and write:
\begin{align*}
    \E_{\x,y\sim P_\theta}\left[ \w^\top \x y \right] = &(v^*_1 + v^*_2)\norm{\mu_c}^2 + \langle \mu_c , v^*_1\bar{\rvn}_1 + v^*_2\bar{\rvn}_2\rangle + \\
    & (v^*_1\theta_1 + v^*_2\theta_2)\theta\norm{\mu_s}^2 + \langle \mu_s, \theta\left(v^*_1\bar{\rvn}_1 + v^*_2\bar{\rvn}_2\right) \rangle \geq \frac{2}{3}(v^*_1 + v^*_2)\norm{\mu_c}^2.
\end{align*}
The inequality follows from the arguments already stated in \lemref{lem:retrieved_solution}, where the second and third items in the above expression have magnitude at most $\frac{1}{6}(v_1^* + v_2^*)\norm{\mu_c}^2$. Now it is left to conclude that $(v_1^* + v_2^*) \geq \frac{\Delta}{2}$, which is a direct consequence of \lemref{lem:v_sum_bound} and \lemref{lem:retrieved_solution}.
\end{proof}

\subsubsection{Proof of \texorpdfstring{\Cref{prop:positive_result_main}}{}} \label{sec:positive_proof_appendix}
Now we are in place to prove the guarantee given in the main paper on the robust error of the model returned by the algorithm. We will restate it here with compatible notation to the earlier parts of this section which slightly differ from those in the main paper (e.g. by incorporating $\Delta$). We also note that to obtain the statement in the main paper we should eliminate the dependence of Assumption ~\ref{ass:norm_constraints_pos_result} on $M_{e,1}$.
We do this by assuming that our algorithm draws $M_{e}$ as half of the original dataset for environment $e$. Then we have that $\sP(M_{e,1} \leq N_{\min} / 8)$ is bounded by  the cumulative probability of a Binomial variable with $k=N_{\min} / 8$ successes and at least $N_{\min}$ trials. This may be bounded with a Hoeffding bound by $1-2 \exp ( \half N_{\min} )$ and with a union bound over the two environments. To absorb this into our failure probability we require $N_{\min} > c_{eo}\log( 1/ \delta)$, leading to this added constraint in the main paper.
\begin{proposition} 
Under \assumref{ass:norm_constraints_pos_result}, let $\epsilon > 0$ be the target maximum error of the model and $t>0$. If $\norm{\mu_c}^2 \geq t Q^{-1}(\epsilon)\frac{15}{\Delta}\sigma^2\sqrt{\frac{d}{N_{\min}}}$, then with probability at least \succesprobpos the robust accuracy error of the model is at most $\epsilon$.
\end{proposition}
\begin{proof}
The error of the model in the environment defined by $\theta\in{[-1, 1]}$ is given by the Gaussian tail function:
\begin{align*}
    Q\left(\frac{\langle \w, \mu_c + \theta\mu_s \rangle}{\sigma\norm{\w}}\right)
\end{align*}
The nominator of this expression is simply the expected score from \lemref{lem:expected_score}, which we already proved is at least $\frac{\Delta}{3}\norm{\mu_c}^2$. Then we need to bound $\norm{\w}$ from above to get a bound on the robust accuracy. According to \corref{corro:positive_result_required_events}, if we denote $N_{\min} = \min\{N_1, N_2 \}$, this upper bound can be taken as $5t\sqrt{\sigma^2 d / N_{\min}}$. We plug this in to get:
\begin{align*}
    \frac{\langle \w, \mu_c + \theta \mu_s \rangle}{\sigma\norm{\w}} \geq \frac{\Delta}{15t}\norm{\mu_c}^2\frac{1}{\sigma^2}\sqrt{\frac{N_{\min}}{d}}
\end{align*}
Since $Q$ is a monotonically decreasing function, if $\norm{\mu_c}^2 \geq t Q^{-1}(\mathrm{\epsilon})\frac{15}{\Delta}\sigma^2\sqrt{\frac{d}{N_{\min}}}$ our model achieves the desired performance.
\end{proof}
